SurfGen: Adversarial 3D Shape Synthesis with Explicit Surface Discriminators

Recent advances in deep generative models have led to immense progress in 3D shape synthesis. While existing models are able to synthesize shapes represented as voxels, point-clouds, or implicit functions, these methods only indirectly enforce the plausibility of the final 3D shape surface. Here we present a 3D shape synthesis framework (SurfGen) that directly applies adversarial training to the object surface. Our approach uses a differentiable spherical projection layer to capture and represent the explicit zero isosurface of an implicit 3D generator as functions defined on the unit sphere. By processing the spherical representation of 3D object surfaces with a spherical CNN in an adversarial setting, our generator can better learn the statistics of natural shape surfaces. We evaluate our model on large-scale shape datasets, and demonstrate that the end-to-end trained model is capable of generating high fidelity 3D shapes with diverse topology.

==> plots/sdf_fig.tex <==
\begin{figure}[t!]

  \includegraphics[width=\linewidth]{plots/sdf_samples.pdf}
  \vspace{-1.5em}
  \caption{On top, we show samples from enforcing only a VAE objective, on the bottom, we show samples which uses our surface discriminator. Thin structures noticeably benefit}
  \vspace{-1.5em}
  \label{fig:render}

\end{figure}

==> plots/sph_proj.tex <==
\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{plots/sph_fig_plot.pdf}
  \vspace{-1.5em}
  \caption{\textbf{(a)-(d)} shows four objects (bottom) and their corresponding depth maps defined (top) when viewed from the side.}
  \vspace{-1.5em}
  \label{fig:sph}

\end{figure}
